Differential Correlation Measurements with the Identity Method

We present an extension of the identity method initially introduced for particle yield fluctuation studies towards measurements of differential correlations. The extension is developed and illustrated in the context of measurements of the normalized two-particle cumulant $R_2$ but is adaptable to any correlation measurements, including differential flow measurements. The identity method is also extended to account for an arbitrary number of particle identification devices and signals.

==> defs.tex <==
\newcommand{ \be }{\begin{linenomath*}\begin{eqnarray}}
\newcommand{ \ee }{\end{eqnarray}\end{linenomath*}}
\newcommand{ \la }{\langle}
\newcommand{ \lla }{\left\langle}
\newcommand{ \ra }{\rangle}
\newcommand{ \rra }{\right\rangle}
\def \mean#1 {{\la #1 \ra}}

\newcommand{ \pp}{p -- p}
\newcommand{ \pPb}{p -- Pb}
\newcommand{ \PbPb}{Pb -- Pb}

\newcommand{ \pvec}{\vec{p}}
\newcommand{ \pvecOne}{\vec{p}_1}
\newcommand{ \pvecTwo}{\vec{p}_2}
\newcommand{ \pt }{p_{\rm T}}
\newcommand{ \ptOne}{p_{\rm T,1}}
\newcommand{ \ptTwo}{p_{\rm T,2}}
\newcommand{ \pti}{p_{\rm T,i}}
\newcommand{ \ptj}{p_{\rm T,j}}
\newcommand{ \ptk}{p_{\rm T,k}}
\newcommand{ \ptik}{p_{\rm T,i,k}}
\newcommand{ \dpt }{dp_{\rm T}}
\newcommand{ \dptOne}{dp_{\rm T,1}}
\newcommand{ \dptTwo}{dp_{\rm T,2}}
\newcommand{ \dpti}{dp_{\rm T,i}}
\newcommand{ \dptj}{dp_{\rm T,j}}
\newcommand{ \Dpt }{\Delta p_{\rm T}}
\newcommand{ \DptDpt }{\Delta \pt \Delta \pt }
\newcommand{ \DeltaPtPt}{\langle  \Delta \pt \Delta \pt \rangle}
\newcommand{ \DptOne}{\Delta p_{\rm T,1}}
\newcommand{ \DptTwo}{\Delta p_{\rm T,2}}
\newcommand{ \dphi}{d\varphi}
\newcommand{ \phiOne}{\varphi_1}
\newcommand{ \phiTwo}{\varphi_2}
\newcommand{ \phii}{\varphi_i}
\newcommand{ \phij}{\varphi_j}
\newcommand{ \dphiOne}{d\varphi_1}
\newcommand{ \dphiTwo}{d\varphi_2}
\newcommand{ \Dphi }{\Delta \varphi}
\newcommand{ \etaOne }{\eta_1}
\newcommand{ \etaTwo }{\eta_2}
\newcommand{ \etai }{\eta_i}
\newcommand{ \etaj }{\eta_j}
\newcommand{ \deta }{d\eta}
\newcommand{ \detaOne }{d\eta_1}
\newcommand{ \detaTwo }{d\eta_2}
\newcommand{ \Deta }{\Delta \eta}
\newcommand{ \etaPhi }{\left( \eta,\varphi \right)}
\newcommand{ \etaPhiI}{\left( \eta_i,\varphi_i\right)}
\newcommand{ \etaPhiOne}{\left( \etaOne,\phiOne\right)}
\newcommand{ \etaPhiTwo}{\left( \etaTwo,\phiTwo\right)}
\newcommand{ \etaPhiPt }{\left( \eta,\varphi,p_t \right)}
\newcommand{ \etaPhiPtI}{\left( \eta_i,\varphi_i,p_{\rm T,i} \right)}
\newcommand{ \etaPhiPtOne}{\left( \etaOne,\phiOne,p_{\rm T,1} \right)}
\newcommand{ \etaPhiPtTwo}{\left( \etaTwo,\phiTwo,p_{\rm T,2} \right)}
\newcommand{ \etaPhiEtaPhi }{\left(  \etaOne,\phiOne,\etaTwo,\phiTwo \right)}
\newcommand{ \etaPhiPtEtaPhiPt }{\left(  \etaOne,\phiOne, p_{\rm T,1}
  \etaTwo,\phiTwo, p_{\rm T,2} \right) } 
\newcommand{ \DetaDphi }{\left(  \Delta \eta, \Delta \varphi \right)}
\newcommand{ \rhoOne}{\rho_1}
\newcommand{ \rhoTwo}{\rho_2}
\newcommand{\Rtwo}{R_2}
\newcommand{\R}{\Rtwo}
\newcommand{\Rpt}{R^{(\Delta p_t)}_2}
\newcommand{\rhoPtPt}{\la p_{\rm T} p_{\rm T} \ra }
%\newcommand{\rhoDptDpt}{R^{\Delta p_t \Delta p_t}_2}
\newcommand{\rhoDptDpt}{\la \Delta p_{\rm T}  \Delta p_{\rm T} \ra }
\newcommand{\rpt}{\Rpt}

\newcommand{ \ds }{\displaystyle}
\newcommand{ \eps}{\varepsilon}
\newcommand{\empha}{et al.}

%========================== COLORS=================
%\definecolor{dgreen}{cmyk}{1.,0.,1.,0.4}        % dark green
\definecolor{dgreen}{cmyk}{1.,0.,1.,0.2}        % dark green
\definecolor{orange}{cmyk}{0.,0.353,1.,0.}    % orange
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{dgreen}{#1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\magenta}[1]{{\color{magenta}{#1}}}
\def \new {\blue}
\def \old {\orange}
\def \ask {\magenta}
\def \snn {\sqrt{s_{_{\rm NN}}}}
\def \bp  {{\bf p}}
\def \mod {{\rm mod}}

